CHoKI-based MPC for blood glucose regulation in Artificial Pancreas

This work presents a Model Predictive Control (MPC) for the artificial pancreas, which is able to autonomously manage basal insulin injections in type 1 diabetic patients. Specifically, the MPC goal is to maintain the patients' blood glucose level inside the safe range of 70-180 mg/dL, acting on the insulin amount and respecting all the imposed constraints, taking into consideration also the Insulin On Board (IOB), to avoid excess of insulin infusion. MPC uses a model to make predictions of the system behaviour. In this work, due to the complexity of the diabetes disease that complicates the identification of a general physiological model, a data-driven learning method is employed instead. The Componentwise H\"{o}lder Kinky Inference (CHoKI) method is adopted, to have a customized controller for each patient. For the data collection phase and also to test the proposed controller, the virtual patients of the FDA-accepted UVA/Padova simulator are exploited. The proposed MPC is also tested on a modified version of the simulator, that takes into consideration also the variability of the insulin sensitivity. The final results are satisfying since the proposed controller reduces the time in hypoglycemia (which is more dangerous) if compared to the outcome obtained with the standard constant basal insulin therapy provided by the simulator, satisfying also the time in range requirements and avoiding long-term hyperglycemia events.

==> 6_results.tex <==
\section{Empirical results}
\label{sec:Empirical_results}
In this Section, we compare the performances of algorithms \GLISprmethod{} and \GLISpmethod{} on a variety of benchmark bound-constrained global optimization problems taken from \cite{Bemporad2020,gramacy2012cases,jamil2013literature,mishra2006some}. Consistently with the preference-based optimization literature, we stick to benchmark problems with less than $n = 10$ decision variables \cite{Bemporad2021,brochu2007active,benavoli2021preferential,gonzalez2017preferential}. %We also consider a different version of the \IDW{} distance function in \eqref{eq:Inverse_distance_weighting_distance_function}, proposed in \cite{zhu2021c} by the same authors, which is equal to:
We also consider the revisited version of the \IDW{} distance function in \eqref{eq:Inverse_distance_weighting_distance_function} employed by \CGLISpmethod{}, which is an extension of \GLISpmethod{} proposed by the same authors\footnote{Note that, in this work, we use \CGLISpmethod{} only to test how the \IDW{} distance function in \eqref{eq:Inverse_distance_weighting_distance_function_C-GLISp} compares to the other formulation in \eqref{eq:Inverse_distance_weighting_distance_function}. However, \CGLISpmethod{} has been developed mainly to extend \GLISpmethod{} in order to handle black-box constraints. The different definition of $z_N\left(\boldsymbol{x}\right)$ is only a minor detail of such paper.}. In particular, in \CGLISpmethod{}:
\begin{align}
    \label{eq:Inverse_distance_weighting_distance_function_C-GLISp}
    z_N(\boldsymbol{x}) = & \left(\frac{N}{N_{max}} - 1\right) \cdot \arctan \left( \frac{\sum_{i = 1, i \neq i_{best}\left( N\right)}^N w_i\left(\boldsymbol{x_{best}}\left(N\right)\right)}{\sum_{i = 1}^N w_i\left(\boldsymbol{x}\right)} \right) + \\
                          & - \frac{N}{N_{max}} \cdot \arctan \left( \frac{1}{\sum_{i = 1}^N w_i\left(\boldsymbol{x}\right)} \right), \quad \forall \boldsymbol{x} \in \mathbb{R}^n \setminus \mathcal{X}, \nonumber
\end{align}
while $z_N(\boldsymbol{x}) = 0, \forall \boldsymbol{x} \in \mathcal{X}$. In \eqref{eq:Inverse_distance_weighting_distance_function_C-GLISp}, $i_{best}\left( N\right) \in \mathbb{N}, 1 \leq i_{best}\left( N\right) \leq N,$ represents the index of the best-found candidate when $\lvert \mathcal{X}\rvert = N$. % $z_N\left(\boldsymbol{x}\right)$ in \eqref{eq:Inverse_distance_weighting_distance_function_C-GLISp} also addresses the shortcomings of the \IDW{} distance function \eqref{eq:Inverse_distance_weighting_distance_function} (analyzed in Section \ref{subsec:Improving_exploration_capabilities_of_GLISp}) which can cause \GLISpmethod{} to get stuck on local minima with no way of escaping. %We will refer to the algorithm that uses \IDW{} distance function in \eqref{eq:Inverse_distance_weighting_distance_function_C-GLISp} as \CGLISpmethod{}.
In practice, $z_N\left(\boldsymbol{x}\right)$ in \eqref{eq:Inverse_distance_weighting_distance_function_C-GLISp} improves the exploratory capabilities of \GLISpmethod{} without the need to define an alternative acquisition function from the one in \eqref{eq:Acquisition_function_GLISp} (see \cite{zhu2021c}).

We point out that we could also consider the preferential Bayesian optimization algorithm in \cite{brochu2007active} as an additional competitor for \GLISprmethod{}. However, in \cite{Bemporad2021}, the authors show that \texttt{GLISp} outperforms the aforementioned method. As we will see in the next Sections, \GLISprmethod{} exhibits convergence speeds that are similar to those of \GLISpmethod{} and hence we have decided to omit the algorithm in \cite{brochu2007active} from our analysis. Moreover, after preliminary testing, the latter method was proven to not be on par w.r.t. the other competitors.

\subsection{Experimental setup}
All benchmark optimization problems have been solved on a machine with two Intel Xeon E5-2687W @3.00GHz CPUs and 128GB of RAM. \GLISprmethod{} has been implemented in MATLAB. Similarly, we have used the MATLAB code for \texttt{GLISp} provided in \cite{Bemporad2021} (formally, version 2.4 of the software package) and the one for \texttt{C-GLISp} supplied in \cite{zhu2021c} (version 3.0 of the same code package). For all the procedures, Problem \eqref{eq:Next_sample_search_no_black-box_constraints} has been solved using Particle Swarm Optimization (\texttt{PSWARM}). In particular, we have used its MATLAB implementation provided by \cite{vaz2007particle,vaz2009pswarm,le2012optimizing}.

To achieve a fair comparison, we have chosen the same hyper-parameters for both \GLISprmethod{} and \GLISpCGLISpmethods{}, whenever possible. This applies, for example, to the shape parameter $\epsilon$, which is initialized to $\epsilon = 1$, and the radial function $\varphi \left(\cdot\right)$, that is an inverse quadratic. Furthermore, the shape parameter for the surrogate model $\hat{f}_N\left(\boldsymbol{x}\right)$ in \eqref{eq:RBF_surrogate_model} is recalibrated using \LOOCV{} (see \GLISpmethod{}) at the iterations  $\mathcal{K}_{R} = \left\{1, 50, 100\right\}$. Its possible values are $\mathcal{E}_{\LOOCV{}} = \{0.1000,$ $0.1668,$ $0.2783,$ $0.4642,$ $0.7743,$ $1,$ $1.2915,$ $2.1544,$ $3.5938,$ $5.9948,$ $10\}$. The remaining hyper-parameters shared by \GLISpCGLISpmethods{} and \GLISprmethod{} are set to $\lambda = 10^{-6}$ and $\sigma = 10^{-2}$. Regarding \GLISprmethod{}, we have chosen $\Delta_{cycle} = \langle 0.95,0.7,0.35,0 \rangle$, where we have included a zero term to comply with the convergence result in Theorem \ref{theo:convergence_of_GLISp-r}. The reasoning behind this cycling sequence is that, after the initial sampling phase, we give priority to the surrogate as to drive the algorithm towards more promising regions of $\Omega$, for example where local minima are located. In practice, if $f\left(\boldsymbol{x}\right)$ is a function that can be approximated well by $\hat{f}_N\left(\boldsymbol{x}\right)$ with little data, starting with a $\delta$ in \eqref{eq:Acquisition_function_GLISp-r} that is close to $1$ might lead the procedure to converge quite faster. If that is not the case, the remaining terms contained inside $\Delta_{cycle}$ promote the exploration of other zones of the constraint set, either dependently or independently from $\hat{f}_N\left(\boldsymbol{x}\right)$. For the sake of completeness, we also analyze the performances of \GLISprmethod{} when equipped with two particular cycling sequences: $\Delta_{cycle} = \langle 0.95 \rangle$ (\quotes{pure} exploitation) and $\Delta_{cycle} = \langle 0 \rangle$ (pure exploration). Concerning \GLISpCGLISpmethods{}, which use $a_N\left(\boldsymbol{x}\right)$ in \eqref{eq:Acquisition_function_GLISp}, we set $\delta = 2$, as proposed by the authors in \cite{Bemporad2021}. Lastly, for \GLISprmethod{}, we select $K_{aug} = 5$ for all optimization problems since, empirically, after several preliminary experiments, it has proven to be good enough to rescale $z_N\left(\boldsymbol{x}\right)$ in \eqref{eq:Inverse_distance_weighting_distance_function} and $\hat{f}_N\left(\boldsymbol{x}\right)$ in \eqref{eq:RBF_surrogate_model} in most cases (see for example \figname{} \ref{fig:Comparison_between_acquisition_function_terms}).
% A summary of the settings used by the algorithms are reported in the supplementary material (\cref{tab:algorithm_settings}).

We run the procedures using a fixed budget of $N_{max}=200$ samples and solve each benchmark optimization problem $N_{trial} = 100$ times, starting from $N_{init} = 4 \cdot n$  points generated by \LHD{}s \cite{mckay2000comparison} with different random seeds. To ensure fairness of comparison, all the algorithms are started from the same samples.

For the sake of clarity, we point out that the preferences between the couples of samples are expressed using the preference function in \eqref{eq:preference_function}, where $f\left(\boldsymbol{x}\right)$ is the corresponding cost function for the considered benchmark optimization problem. Therefore, the preferences are always expressed consistently, allowing us to compare \GLISprmethod{} and \GLISpCGLISpmethods{} properly. That would not necessarily be the case if a human decision-maker was involved.

\subsection{Results}
We compare the performances of \GLISprmethod{} and \GLISpCGLISpmethods{} on each benchmark optimization problem by means of \important{convergence plots} and \important{data profiles} \cite{audet2017derivative}. Convergence plots depict the median, best and worst case performances over the $N_{trial}$ instances and with respect to the cost function values achieved by $\boldsymbol{x_{best}}\left(N\right)$, as $N$ increases. Data profiles are one of the most popular tools for assessing efficiency and robustness of global optimization methods: efficient surrogate-based methods exhibit steep slopes (i.e. fast convergences speeds), while robust algorithms are able to solve more (instances of) problems within the budget $N_{max}$. In general, no method is both efficient and robust: a trade-off must be made \cite{thanedar1990robustness}. Typically, data profiles are used to visualize the performances of several algorithms on multiple benchmark optimization problems simultaneously. However, due to the stochastic nature of \LHD{}s \cite{mckay2000comparison}, here we will also depict the data profiles for \GLISprmethod{}, \GLISpmethod{} and \CGLISpmethod{} on each benchmark optimization problem on its own, highlighting how the algorithms behave when started from different samples. In practice, data profiles show, for $1 \leq N \leq N_{max}$, how many among the $N_{trial}$ instances of one (or several) benchmark optimization problem(s) have been solved to a prescribed \important{accuracy}, defined as \cite{audet2017derivative}:
\begin{equation}
    \label{eq:accuracy}
    acc\left(N\right) = \frac{f\left(\boldsymbol{x_{best}}\left(N\right)\right)-f\left(\boldsymbol{x}_{1}\right)}{f^*-f\left(\boldsymbol{x}_{1}\right)},
\end{equation}
where $f^* = \min{\boldsymbol{x} \in \Omega} f\left(\boldsymbol{x}\right)$. In particular, here we consider a benchmark optimization problem to be solved by some algorithm when $acc\left(N\right) > t, t = 0.95$. In what follows, the results achieved by \GLISprmethod{} equipped with $\Delta_{cycle} = \langle 0.95 \rangle$ and $\Delta_{cycle} = \langle 0 \rangle$ are reported only in the data profiles (and not in the convergence plots), to make the graphs more readable.

\figname{} \ref{fig:cumulative_data_profiles} shows the cumulative data profiles of \GLISprmethod{}, \GLISpmethod{} and \CGLISpmethod{}, which result from considering all the benchmark optimization problems simultaneously. Instead, \figname{} \ref{fig:performances_on_benchmarks_1} and \figname{} \ref{fig:performances_on_benchmarks_2} depict the convergence plots and the data profiles achieved by the considered algorithms on each benchmark. In \tablename{} \ref{tab:algorithm_comparison} we report the number of samples required to reach the accuracy $t = 0.95$, i.e.:
\begin{equation}
    \label{eq:number_of_samples_for_relative_accuracy}
    N_{acc > t} = \min{1 \leq N \leq N_{max}} N \quad \text{ such that } acc\left(N\right) > t.
\end{equation}
In practice, given that each benchmark optimization problem is solved multiple times, $N_{acc > t}$ in \tablename{} \ref{tab:algorithm_comparison} is assessed median-wise (over the $N_{trial}$ instances), giving us an indication on the efficiency of each method. In the same Table, we also report the percentages of instances of problems solved by \GLISprmethod{}, \GLISpmethod{} and \CGLISpmethod{} (which is an indicator of robustness) and the average execution times of each algorithm.

From our experiments, we gather that:
\begin{itemize}
    \item \important{\GLISprmethod{} ($\Delta_{cycle} = \langle 0.95, 0.7, 0.35, 0\rangle$) can be notably more robust than \GLISpmethod{} without excessively compromising its convergence speed}. On several occasions, the latter algorithm gets stuck on local minima of the benchmark optimization problems. That is particularly evident on the \bemporadGOP{} and \gramacyandleeGOP{} benchmarks, in which cases \GLISpmethod{} solves, respectively, only $70\%$ and $31\%$ of the $N_{trial}$ instances. Instead, \GLISprmethod{} ($\Delta_{cycle} = \langle 0.95, 0.7, 0.35, 0\rangle$) is able to solve both of them to the prescribed accuracy. % As further proof, the best candidates found by all the considered procedures when solving the \gramacyandleeGOP{} benchmark are depicted in Figure \ref{fig:gramacy_and_lee_benchmark}. In this case, $f\left(\boldsymbol{x}\right)$ is highly multimodal and \GLISpmethod{} often fails to find the global minimizer $\boldsymbol{x^*}$. That is due to the shortcomings of $z_N\left(\boldsymbol{x}\right)$ in \eqref{eq:Inverse_distance_weighting_distance_function} (see  Section \ref{subsec:Improving_exploration_capabilities_of_GLISp}), which compromise the exploratory capabilities of the method. As a matter of fact, on the \gramacyandleeGOP{} benchmark, even \GLISprmethod{} with $\Delta_{cycle} = \langle 0 \rangle$ (pure exploration) converges to $\boldsymbol{x^*}$ relatively quickly. 
          In practice, \GLISpmethod{} shines when exploitation is better suited for the benchmark optimization problem at hand. That is particularly relevant for the \bukinsixGOP{} problem, on which both \GLISpmethod{} and \GLISprmethod{} with $\Delta_{cycle} = \langle 0.95 \rangle$  (\quotes{pure} exploitation) perform quite well. Lastly, \CGLISpmethod{} is as robust as \GLISprmethod{} ($\Delta_{cycle} = \langle 0.95, 0.7, 0.35, 0\rangle$) but is the least efficient among the analyzed procedures.
    \item The pure exploration strategy (i.e. \GLISprmethod{} with $\Delta_{cycle} = \langle 0\rangle$) performs poorly, even for $n = 2$. When $n = 5$, it is unable solve any problem (in fact, the data profiles stay flat after the initial sampling phase). Only for $n = 1$ the pure exploration strategy is quite robust and relatively efficient.
    \item Vice-versa, a \quotes{pure} exploitatory approach (i.e. \GLISprmethod{} with $\Delta_{cycle} = \langle 0.95\rangle$), although not necessarily globally convergent (see Theorem \ref{theo:convergence_of_GLISp-r}), can actually be successful on some benchmark optimization problems. Often, such strategy exhibits a slightly lower $N_{acc > t}$ (median-wise) than the other procedures, see Table \ref{tab:algorithm_comparison}. Notably, the data profiles of \GLISprmethod{} ($\Delta_{cycle} = \langle 0.95\rangle$) can be quite similar to those of \GLISpmethod{}. Therefore, we could say that \GLISpmethod{} has limited exploratory capabilities. %(again, this is to be attributed to the shortcomings of $z_N\left(\boldsymbol{x}\right)$ in \eqref{eq:Inverse_distance_weighting_distance_function}, described in Section \ref{subsec:Improving_exploration_capabilities_of_GLISp}).
    \item The main disadvantage of \GLISprmethod{}, compared to \GLISpmethod{} and \CGLISpmethod{}, is the increased computational time, as reported in Table \ref{tab:algorithm_comparison}. That is due to the computational overhead of Algorithm \ref{alg:Augmented_sample_set}, which generates the augmented sample set $\mathcal{X}_{aug}$ for the proposed procedure by performing $K$-means clustering. On average, \GLISprmethod{} ($\Delta_{cycle} = \langle 0.95, 0.7, 0.35, 0\rangle$) is $31\%$ slower than \GLISpmethod{} and $72\%$ slower than \CGLISpmethod{}. However, we point out that these overheads are practically negligible when the queries to the decision-maker involve running computer simulations or performing real-world experiments which, contrary to the considered benchmark optimization problems, can take from a few minutes up to several hours. This is a common  assumption made by surrogate-based methods: at each iteration, the most time-consuming operation is the query to the decision-maker (or, in the context of black-box optimization, the measure of the cost function \cite{vu2017surrogate,jones2001taxonomy}).
\end{itemize}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\textwidth]{cumulative_data_profile}

    \caption{
        \label{fig:cumulative_data_profiles}
        Cumulative data profiles ($acc\left(N\right) > 95\%$) %that show the overall performances achieved by 
        of the considered preference-based optimization algorithms. \GLISprmethod{} is depicted in red ($\Delta_{cycle} = \langle 0.95, 0.7, 0.35, 0\rangle$ continuous line, $\Delta_{cycle} = \langle 0.95 \rangle$ dashed line, $\Delta_{cycle} = \langle 0 \rangle$ dotted line), \GLISpmethod{} in blue and \CGLISpmethod{} in green.
    }
\end{figure}

% \input{9_figures_and_tables_for_results.tex}

==> 7_discussion.tex <==
\section{Conclusions}
\label{sec:Discussion}
In this work, we introduced the preference-based optimization problem from a utility theory perspective. Then, we extended algorithm \GLISpmethod{}, giving rise \GLISprmethod{}. In particular, we have addressed the shortcomings of $a_N\left(\boldsymbol{x}\right)$ in \eqref{eq:Acquisition_function_GLISp}, defined a new acquisition function and proposed the greedy $\delta$-cycling strategy, which dynamically varies the exploration-exploitation weight $\delta$ in \eqref{eq:Acquisition_function_GLISp-r}. %Many black-box optimization algorithms follow this rationale of alternating between local and global search, however no such strategy has been employed in \GLISpmethod{}. 
Furthermore, we have proven the global convergence of \GLISprmethod{}, which is strictly related to the choice of the cycling sequence $\Delta_{cycle}$. To the best of our knowledge, \GLISprmethod{} is the first preference-based surrogate-based method with a formal proof of convergence.

Compared to the original method, the proposed extension is less likely to get stuck on local minima of the scoring function and proves to be more robust on several benchmark optimization problems without particularly compromising its convergence speed. Moreover, we have also considered algorithm \CGLISpmethod{}, which %overcomes the limitations of $z_N\left(\boldsymbol{x}\right)$ in \eqref{eq:Inverse_distance_weighting_distance_function} 
improves the exploratory capabilities of \GLISpmethod{} by employing a different exploration function. In our experiments, we have observed that, even though \CGLISpmethod{} is as robust as \GLISprmethod{}, it often exhibits slower convergence rates compared to \GLISpmethod{} and the proposed extension.

Further research is devoted to extending \GLISprmethod{} in order to handle black-box constraints, which involve functions whose analytical formulations are not available. One possibility is to follow the same reasoning behind \CGLISpmethod{}, which does so by adding a term to the acquisition function that penalizes the exploration in those regions of $\Omega$ where the black-box constraints are likely to be violated. Additionally, a compelling line of research concerns preference-based optimization problems in the case where the human decision-maker is \quotes{irrational} (in a sense that some of the properties in Definition \ref{def:rational_decision_maker}, typically completeness, do not hold). From a practical perspective, when the preference relation $\succsim$ on $\Omega$ of the \DM{} is not complete, we would need a surrogate model that is able to handle the answer \quotes{I do not know} when the decision-maker cannot decide which, among two calibrations, he/she prefers.

\paragraph*{Data availability} The benchmark optimization problems considered in Section \ref{sec:Empirical_results} are reported in \cite{Bemporad2020,gramacy2012cases,jamil2013literature,mishra2006some}. The MATLAB code for algorithms \GLISpmethod{} and \CGLISpmethod{} is provided in the corresponding papers. The MATLAB code for the proposed method, \GLISprmethod{}, is supplied in the supplementary material provided in \cite{previtali2023glisp}.

==> 8_statements_and_declarations.tex <==
\subsubsection*{Statements and declarations}
\paragraph*{Conflict of interest} All the authors declare that they have no conflict of interest.

==> 9_figures_and_tables_for_results.tex <==
% Report the figures and the tables that concern the empirical results at the end, to save space
\begin{figure}[!htb]
    \centering
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{bemporad_n_1_MC.png}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{bemporad_n_1_MC_pp}
    }

    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{gramacy_and_lee_n_1_MC}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{gramacy_and_lee_n_1_MC_pp}
    }

    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{ackley_n_2_MC}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{ackley_n_2_MC_pp}
    }

    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{bukin_6_n_2_MC}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{bukin_6_n_2_MC_pp}
    }

    \caption{
        \label{fig:performances_on_benchmarks_1}
        Performances achieved by the considered preference-based optimization algorithms on the benchmark optimization problems: convergence plots on the left and data profiles ($acc\left(N\right) > 95\%$) on the right. \GLISprmethod{} (with $\Delta_{cycle} = \langle 0.95, 0.7, 0.35, 0\rangle$) is depicted in red, \GLISpmethod{} in blue and \CGLISpmethod{} in green. The dashed black-line in the convergence plots represents $f^*$. We also show the number of initial samples, $N_{init}$, with a black vertical line. The results obtained by \GLISprmethod{} with $\Delta_{cycle} = \langle 0.95\rangle$ (dashed red line) and \GLISprmethod{} with $\Delta_{cycle} = \langle 0\rangle$ (dotted red line) are shown only in the data profiles.
    }
\end{figure}

\begin{figure}[!htb]
    \centering
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{levi_13_n_2_MC}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{levi_13_n_2_MC_pp}
    }

    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{adjiman_n_2_MC}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{adjiman_n_2_MC_pp}
    }

    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{rosenbrock_n_5_MC}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{rosenbrock_n_5_MC_pp}
    }

    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{step_n_5_MC}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{step_n_5_MC_pp}
    }

    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{salomon_n_5_MC}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{salomon_n_5_MC_pp}
    }

    \caption{
        \label{fig:performances_on_benchmarks_2}
        \figname{} \ref{fig:performances_on_benchmarks_1} cont'd.
    }
\end{figure}

\begin{comment}
    \begin{figure}[!htb]
    \centering
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{C-GLISp-r regular - Best sample for each simulation}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{C-GLISp-r exploitation - Best sample for each simulation}
    }

    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{C-GLISp-r exploration - Best sample for each simulation}
    }
    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{GLISp - Best sample for each simulation}
    }

    \subfloat{
        \centering
        \includegraphics[width=.5\textwidth]{C-GLISp - Best sample for each simulation}
    }

    \caption{
        \label{fig:gramacy_and_lee_benchmark}
        Best samples found by the considered preference-based optimization procedures on the \gramacyandleeGOP{} benchmark. Each point in magenta represents $x_{best}\left(N_{max}\right)$ for the corresponding instance. The blue star depicts the global minimizer of the benchmark optimization problem.
    }
\end{figure}
\end{comment}

\begin{comment}
\begin{sidewaystable}[!htb]
    \sidewaystablefn%
    \settablestretch
    \settablefontsize
    \caption{
        \label{tab:median_accuracies}
        Number of samples required by the considered algorithms to solve the benchmark optimization problems to an accuracy of $0.95$ (median-wise). The acronym \texttt{n.r.} stands for \quotes{not reached}. The best results are highlighted in bold font.
    }
    \centering
    %\colorrowsoftable{13}
    \begin{tabular}{ccccccc}
        \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7}
                                                    &                      & \multicolumn{5}{c}{$N_{acc>0.95}$}\tabularnewline
        \hline
        \multirow{2}{*}{\textbf{Benchmark problem}} & \multirow{2}{*}{$n$} & \multirow{2}{*}{\GLISpmethod{}}                   & \multirow{2}{*}{\CGLISpmethod{}} & \multicolumn{3}{c}{\GLISprmethod{}}\tabularnewline
        \cline{5-7} \cline{6-7} \cline{7-7}
                                                    &                      &                                                   &                                  & $\Delta_{cycle}=\langle0.95,0.7,0.35,0\rangle$     & $\Delta_{cycle}=\langle0.95\rangle$ & $\Delta_{cycle}=\langle0\rangle$\tabularnewline
        \hline
        \multirow{1}{*}{\bemporadGOP}               & \multirow{1}{*}{$1$} & $\boldsymbol{8}$                                  & $15$                             & $11$                                               & $\boldsymbol{8}$                    & $18$\tabularnewline
        %\colorrowoftable 
        \multirow{1}{*}{\gramacyandleeGOP{}}        & \multirow{1}{*}{$1$} & \texttt{n.r.}                                     & $32$                             & $\boldsymbol{31}$                                  & \texttt{n.r.}                       & $36$\tabularnewline
        \multirow{1}{*}{\ackleyGOP{}}               & \multirow{1}{*}{$2$} & \texttt{n.r.}                                     & \texttt{n.r.}                    & \texttt{n.r.}                                      & \texttt{n.r.}                       & \texttt{n.r.}\tabularnewline
        %\colorrowoftable 
        \multirow{1}{*}{\bukinsixGOP{}}             & \multirow{1}{*}{$2$} & $24$                                              & $193$                            & $58$                                               & $\boldsymbol{23}$                   & \texttt{n.r.}\tabularnewline
        \multirow{1}{*}{\levythirteenGOP{}}         & \multirow{1}{*}{$2$} & $\boldsymbol{9}$                                  & $22$                             & $\boldsymbol{9}$                                   & $\boldsymbol{9}$                    & $34$\tabularnewline
        %\colorrowoftable
        \multirow{1}{*}{\adjimanGOP{}}              & \multirow{1}{*}{$2$} & $\boldsymbol{11}$                                 & $15$                             & $12$                                               & $12$                                & $24$\tabularnewline
        %\multirow{1}{*}{\texttt{camel three hump}}  & \multirow{1}{*}{$2$} & $\boldsymbol{9}$                                  & $\boldsymbol{9}$                  & $\boldsymbol{9}$                                    & $\boldsymbol{9}$                    & $13$\tabularnewline
        \multirow{1}{*}{\rosenbrockGOP{}}           & \multirow{1}{*}{$5$} & $\boldsymbol{21}$                                 & $26$                             & $\boldsymbol{21}$                                  & $\boldsymbol{21}$                   & \texttt{n.r.}\tabularnewline
        %\colorrowoftable 
        \multirow{1}{*}{\steptwoGOP{}}              & \multirow{1}{*}{$5$} & $\boldsymbol{22}$                                 & $100$                            & $\boldsymbol{22}$                                  & $\boldsymbol{22}$                   & \texttt{n.r.}\tabularnewline
        \multirow{1}{*}{\salomonGOP{}}              & \multirow{1}{*}{$5$} & \texttt{n.r.}                                     & \texttt{n.r.}                    & \texttt{n.r.}                                      & \texttt{n.r.}                       & \texttt{n.r.}\tabularnewline
        \hline
        \tabularnewline % Leave some space for next table
    \end{tabular}
\end{sidewaystable}

\begin{sidewaystable}[!htb]
    \sidewaystablefn%
    \settablestretch
    \settablefontsize
    \caption{
        \label{tab:average_execution_times}
        Average execution times of the considered algorithms. The best results are highlighted in bold font.
    }
    \centering
    % \colorrowsoftable{13}
    \begin{tabular}{ccccccc}
        \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7}
                                                    &                      & \multicolumn{5}{c}{\textbf{Average execution times} $[sec]$}\tabularnewline
        \hline
        \multirow{2}{*}{\textbf{Benchmark problem}} & \multirow{2}{*}{$n$} & \multirow{2}{*}{\GLISpmethod{}}                                             & \multirow{2}{*}{\CGLISpmethod{}} & \multicolumn{3}{c}{\GLISprmethod{}}\tabularnewline
        \cline{5-7} \cline{6-7} \cline{7-7}
                                                    &                      &                                                                             &                                  & $\Delta_{cycle}=\langle0.95,0.7,0.35,0\rangle$     & $\Delta_{cycle}=\langle0.95\rangle$ & $\Delta_{cycle}=\langle0\rangle$\tabularnewline
        \hline \bemporadGOP{}                       & $1$                  & $79.8$                                                                      & $\boldsymbol{57.5}$              & $79.4$                                             & $109.7$                             & $71.4$\tabularnewline
        \gramacyandleeGOP{}                         & $1$                  & $74.4$                                                                      & $\boldsymbol{58.1}$              & $67.5$                                             & $90.8$                              & $63.8$\tabularnewline
        \ackleyGOP{}                                & $2$                  & $92.1$                                                                      & $\boldsymbol{70.3}$              & $127.9$                                            & $122.4$                             & $121.1$\tabularnewline
        \bukinsixGOP{}                              & $2$                  & $84.5$                                                                      & $\boldsymbol{73.3}$              & $115.0$                                            & $114.6$                             & $123.6$\tabularnewline
        \levythirteenGOP{}                          & $2$                  & $82.0$                                                                      & $\boldsymbol{69.3}$              & $126.8$                                            & $118.2$                             & $120.6$\tabularnewline
        \adjimanGOP{}                               & $2$                  & $105.4$                                                                     & $\boldsymbol{71.6}$              & $146.1$                                            & $124.0$                             & $117.5$\tabularnewline
        %\texttt{camel three hump} & $2$ & $83.6$ & $\boldsymbol{70.1}$ & $132.5$ & $113.3$ & $123.7$\tabularnewline
        \rosenbrockGOP{}                            & $5$                  & $133.3$                                                                     & $107.1$                          & $190.2$                                            & $222.3$                             & $\boldsymbol{100.2}$\tabularnewline
        \steptwoGOP{}                               & $5$                  & $148.1$                                                                     & $104.2$                          & $190.6$                                            & $216.7$                             & $\boldsymbol{98.9}$\tabularnewline
        \salomonGOP{}                               & $5$                  & $137.7$                                                                     & $103.5$                          & $183.4$                                            & $219.1$                             & $\boldsymbol{100.8}$\tabularnewline
        \hline
    \end{tabular}
\end{sidewaystable}
\end{comment}

\begin{sidewaystable}[!htb]
    %\sidewaystablefn%
    \settablestretch
    \settablefontsize
    \caption{
        \label{tab:algorithm_comparison}
        Comparison between the considered preference-based optimization algorithms. Several indicators are taken into account: (a) \important{efficiency indicator}, i.e. number of samples required to solve the benchmark optimization problems to an accuracy of $0.95$ (median-wise), as defined in \eqref{eq:number_of_samples_for_relative_accuracy}, (b) \important{robustness indicator}, i.e. percentage of (instances of) problems solved and (c) average execution times (in seconds). The acronym \texttt{n.r.} stands for \quotes{not reached}. The best results are highlighted in bold font. We also report the average performances over all the considered benchmark optimization problems. Note that the averages for indicator (a) do not consider those benchmarks for which the algorithms did not reach the desired accuracy. %and thus should be taken with a grain of salt.
    }
    \centering
    % \colorrowsoftable{13}
    \begin{tabular}{cc|ccc|ccc|ccc|ccc|ccc}
        \multicolumn{8}{c}{}                  & \multicolumn{9}{c}{\GLISprmethod{}}\tabularnewline
        \cline{9-17} \cline{10-17} \cline{11-17} \cline{12-17} \cline{13-17} \cline{14-17} \cline{15-17} \cline{16-17} \cline{17-17}
        \multicolumn{2}{c|}{}                 & \multicolumn{3}{c|}{\GLISpmethod{}}                & \multicolumn{3}{c|}{\CGLISpmethod{}} & \multicolumn{3}{c|}{$\Delta_{cycle}=\langle0.95,0.7,0.35,0\rangle$} & \multicolumn{3}{c|}{$\Delta_{cycle}=\langle0.95\rangle$} & \multicolumn{3}{c}{$\Delta_{cycle}=\langle0\rangle$}\tabularnewline
        \hline
        \textbf{Benchmark}                    & \multirow{1}{*}{$n$}                               & (a)                                  & (b)                                                                 & (c)                                                      & (a)                                                                 & (b)                  & (c)                 & (a)                   & (b)                  & (c)                 & (a)               & (b)                  & (c)     & (a)           & (b)                    & (c)\tabularnewline
        \hline
        \bemporadGOP{}                        & $1$                                                & $\boldsymbol{8}$                     & $70\%$                                                              & $79.8$                                                   & $15$                                                                & $\boldsymbol{100\%}$ & $\boldsymbol{57.5}$ & $11$                  & $\boldsymbol{100\%}$ & $79.4$              & $\boldsymbol{8}$  & $68\%$               & $109.7$ & $18$          & $\boldsymbol{100\%}$   & $71.4$\tabularnewline
        \multirow{1}{*}{\gramacyandleeGOP{}}  & \multirow{1}{*}{$1$}                               & \texttt{n.r.}                        & $31\%$                                                              & $74.4$                                                   & $32$                                                                & $\boldsymbol{100\%}$ & $\boldsymbol{58.1}$ & $\boldsymbol{31}$     & $\boldsymbol{100\%}$ & $67.5$              & \texttt{n.r.}     & $30\%$               & $90.8$  & $36$          & $99\%$                 & $63.8$\tabularnewline
        \multirow{1}{*}{\ackleyGOP{}}         & \multirow{1}{*}{$2$}                               & \texttt{n.r.}                        & $24\%$                                                              & $92.1$                                                   & \texttt{n.r.}                                                       & $8\%$                & $\boldsymbol{70.3}$ & \texttt{n.r.}         & $\boldsymbol{28\%}$  & $127.9$             & \texttt{n.r.}     & $17\%$               & $122.4$ & \texttt{n.r.} & $1\%$                  & $121.1$\tabularnewline
        \multirow{1}{*}{\bukinsixGOP{}}       & \multirow{1}{*}{$2$}                               & $24$                                 & $\boldsymbol{99\%}$                                                 & $84.5$                                                   & $193$                                                               & $60\%$               & $\boldsymbol{73.3}$ & $58$                  & $78\%$               & $115.0$             & $\boldsymbol{23}$ & $98\%$               & $114.6$ & \texttt{n.r.} & $16\%$                 & $123.6$\tabularnewline
        \multirow{1}{*}{\levythirteenGOP{}}   & \multirow{1}{*}{$2$}                               & $\boldsymbol{9}$                     & $97\%$                                                              & $82.0$                                                   & $22$                                                                & $\boldsymbol{100\%}$ & $\boldsymbol{69.3}$ & $\boldsymbol{9}$      & $99\%$               & $126.8$             & $\boldsymbol{9}$  & $84\%$               & $118.2$ & $34$          & $91\%$                 & $120.6$\tabularnewline
        \multirow{1}{*}{\adjimanGOP{}}        & \multirow{1}{*}{$2$}                               & $\boldsymbol{11}$                    & $97\%$                                                              & $105.4$                                                  & $15$                                                                & $\boldsymbol{100\%}$ & $\boldsymbol{71.6}$ & $12$                  & $\boldsymbol{100\%}$ & $146.1$             & $12$              & $\boldsymbol{100\%}$ & $124.0$ & $24$          & $99\%$                 & $117.5$\tabularnewline
        \multirow{1}{*}{\rosenbrockGOP{}}     & \multirow{1}{*}{$5$}                               & $\boldsymbol{21}$                    & $\boldsymbol{100\%}$                                                & $133.3$                                                  & $26$                                                                & $\boldsymbol{100\%}$ & $107.1$             & $\boldsymbol{21}$     & $\boldsymbol{100\%}$ & $190.2$             & $\boldsymbol{21}$ & $\boldsymbol{100\%}$ & $222.3$ & \texttt{n.r.} & $41\%$                 & $\boldsymbol{100.2}$\tabularnewline
        \multirow{1}{*}{\steptwoGOP{}}        & \multirow{1}{*}{$5$}                               & $\boldsymbol{22}$                    & $\boldsymbol{100\%}$                                                & $148.1$                                                  & $100$                                                               & $\boldsymbol{100\%}$ & $104.2$             & $\boldsymbol{22}$     & $\boldsymbol{100\%}$ & $190.6$             & $\boldsymbol{22}$ & $\boldsymbol{100\%}$ & $216.7$ & \texttt{n.r.} & $3\%$                  & $\boldsymbol{98.9}$\tabularnewline
        \salomonGOP{}                         & $5$                                                & \texttt{n.r.}                        & $\boldsymbol{18\%}$                                                 & $137.7$                                                  & \texttt{n.r.}                                                       & $17\%$               & $103.5$             & \texttt{n.r.}         & $14\%$               & $183.4$             & \texttt{n.r.}     & $16\%$               & $219.1$ & \texttt{n.r.} & $0\%$                  & $\boldsymbol{100.8}$\tabularnewline
        \hline
        \multicolumn{2}{c|}{\textbf{Average}} & $\boldsymbol{15.8}$                                & $70.7\%$                             & $104.1$                                                             & $57.6$                                                   & $76.1\%$                                                            & $\boldsymbol{79.4}$  & $23.4$              & $\boldsymbol{79.8\%}$ & $136.3$              & $\boldsymbol{15.8}$ & $68.1\%$          & $148.6$              & $28.0$  & $56.3\%$      & $102.0$\tabularnewline
    \end{tabular}
\end{sidewaystable}

==> A_proofs.tex <==
\section{Additional proofs}
\label{sec:additional_proofs}
\paragraph*{Proof of Lemma \ref{lemma:Gradient_of_IDW_distance_function}}
The \IDW{} distance function in \eqref{eq:Inverse_distance_weighting_distance_function} is differentiable at any $\boldsymbol{x} \in \mathbb{R}^{n}$ (see Proposition \ref{prop:Differentiability_of_IDW_distance_function}); thus, its gradient $\nabla _{\boldsymbol{x}} z_N\left(\boldsymbol{x}\right)$ is defined everywhere and can be computed by repeatedly applying the chain rule.

Consider the case $\boldsymbol{x} \in \mathbb{R}^n \setminus \mathcal{X}$. First of all, it is easy to prove that the \IDW{} function $w_{i}\left(\boldsymbol{x}\right)$ in \eqref{eq:Inverse_distance_weighting_function} is differentiable at any $\boldsymbol{x} \in \mathbb{R}^{n}\setminus\left\{ \boldsymbol{x}_{i}\right\}$. That is because the squared Euclidean norm $\euclideannorm{\boldsymbol{x}-\boldsymbol{x}_{i}}^2$ is differentiable everywhere and also:
\begin{equation*}
    \euclideannorm{\boldsymbol{x}-\boldsymbol{x}_{i}}^2 \neq 0, \quad \forall \boldsymbol{x} \in \mathbb{R}^{n}\setminus\left\{\boldsymbol{x}_{i}\right\}.
\end{equation*}
Therefore, due to the reciprocal rule, the \IDW{} function is differentiable at any $\boldsymbol{x} \in \mathbb{R}^{n}\setminus\left\{\boldsymbol{x}_{i}\right\}$. In order to compute the gradient of $w_{i}\left(\boldsymbol{x}\right)$ in \eqref{eq:Inverse_distance_weighting_function}, recall that the gradient of the squared Euclidean norm is equal to:
\begin{equation}
    \label{eq:Gradient_of_Euclidean_Norm}
    \nabla_{\boldsymbol{x}}\euclideannorm{\boldsymbol{x}-\boldsymbol{x}_{i}}^2 = 2\cdot\left(\boldsymbol{x}-\boldsymbol{x}_{i}\right), \quad \forall \boldsymbol{x} \in \mathbb{R}^n.
\end{equation}
%Now, let $\boldsymbol{x} \in \mathbb{R}^{n}\setminus\left\{ \boldsymbol{x}_{i}\right\}$. 
Using \eqref{eq:Gradient_of_Euclidean_Norm}, it is easy to prove that:
\begin{align}
    \label{eq:Gradient_of_IDW_function}
    \nabla_{\boldsymbol{x}}w_{i}\left(\boldsymbol{x}\right) & =-2\cdot\frac{\boldsymbol{x}-\boldsymbol{x}_{i}}{\euclideannorm{\boldsymbol{x}-\boldsymbol{x}_{i}}^{4}} \nonumber                                                                             \\
                                                            & =-2\cdot\left(\boldsymbol{x}-\boldsymbol{x}_{i}\right)\cdot w_{i}\left(\boldsymbol{x}\right)^{2}, \quad \forall \boldsymbol{x} \in \mathbb{R}^{n}\setminus\left\{ \boldsymbol{x}_{i}\right\}.
\end{align}
Now, let us consider the argument of the $\arctan \left(\cdot\right)$ function in $z_N\left(\boldsymbol{x}\right)$, which is (see \eqref{eq:Inverse_distance_weighting_distance_function}):
\begin{equation*}
    \label{eq:Reciprocal_of_sum_of_IDW_functions}
    h\left(\boldsymbol{x}\right) = \frac{1}{\sum_{i=1}^{N}w_{i}\left(\boldsymbol{x}\right)}, \quad \forall \boldsymbol{x} \in \mathbb{R}^n \setminus \mathcal{X}.
\end{equation*}
We can find the gradient of $h\left(\boldsymbol{x}\right)$ by applying the chain rule in combination with \eqref{eq:Gradient_of_IDW_function}:
\begin{equation}
    \label{eq:Gradient_of_reciprocal_of_sum_of_IDW_functions}
    \nabla_{\boldsymbol{x}}h\left(\boldsymbol{x}\right) =2\cdot\frac{\sum_{i=1}^{N}\left(\boldsymbol{x}-\boldsymbol{x}_{i}\right)\cdot w_{i}\left(\boldsymbol{x}\right)^{2}}{\left[\sum_{i=1}^{N}w_{i}\left(\boldsymbol{x}\right)\right]^{2}},
    \quad \forall \boldsymbol{x} \in \mathbb{R}^{n} \setminus \mathcal{X}.
\end{equation}
Finally, using \eqref{eq:Gradient_of_reciprocal_of_sum_of_IDW_functions} and applying the chain rule one last time, we can compute the gradient of the \IDW{} distance function in \eqref{eq:Inverse_distance_weighting_distance_function}:
\begin{align}
    \label{eq:Inverse_distance_weighting_distance_function_gradient_partial_1}
    \nabla_{\boldsymbol{x}}z_N\left(\boldsymbol{x}\right) & =\frac{d}{dt} \left[-\frac{2}{\pi}\cdot \arctan\left(t\right)\right]\evaluatedat{t=h\left(\boldsymbol{x}\right)}\cdot\nabla_{\boldsymbol{x}}h\left(\boldsymbol{x}\right) \nonumber                                                                                                            \\
    % &=-\frac{4}{\pi}\cdot\frac{1}{1+\left[\frac{1}{\sum_{i=1}^{N}w_{i}\left(\boldsymbol{x}\right)}\right]^{2}}\cdot\frac{\sum_{i=1}^{N}\left(\boldsymbol{x}-\boldsymbol{x}_{i}\right)\cdot w_{i}\left(\boldsymbol{x}\right)^{2}}{\left[\sum_{i=1}^{N}w_{i}\left(\boldsymbol{x}\right)\right]^{2}} \nonumber \\
                                                          & =-\frac{4}{\pi}\cdot\frac{1}{1+\left[\sum_{i=1}^{N}w_{i}\left(\boldsymbol{x}\right)\right]^{-2}}\cdot\frac{\sum_{i=1}^{N}\left(\boldsymbol{x}-\boldsymbol{x}_{i}\right)\cdot w_{i}\left(\boldsymbol{x}\right)^{2}}{\left[\sum_{i=1}^{N}w_{i}\left(\boldsymbol{x}\right)\right]^{2}} \nonumber \\                                        & =-\frac{4}{\pi}\cdot\frac{\sum_{i=1}^{N}\left(\boldsymbol{x}-\boldsymbol{x}_{i}\right)\cdot w_{i}\left(\boldsymbol{x}\right)^{2}}{1+\left[\sum_{i=1}^{N}w_{i}\left(\boldsymbol{x}\right)\right]^{2}}, \quad
    \forall \boldsymbol{x} \in \mathbb{R}^{n} \setminus \mathcal{X}.
\end{align}
Now, let us consider the case $\boldsymbol{x}_i \in \mathcal{X}$. In \cite{Bemporad2020}, the authors have proven that all the partial derivatives of $z_N\left(\boldsymbol{x}\right)$ in \eqref{eq:Inverse_distance_weighting_distance_function} are zero at each $\boldsymbol{x}_i \in \mathcal{X}$, i.e.
\begin{equation}
    \label{eq:Inverse_distance_weighting_distance_function_gradient_partial_2}
    \nabla_{\boldsymbol{x}}z_N\left(\boldsymbol{x}_i\right) = \boldsymbol{0}_{n}, \quad \forall \boldsymbol{x}_i \in \mathcal{X}.
\end{equation}
Lastly, combining \eqref{eq:Inverse_distance_weighting_distance_function_gradient_partial_1} and \eqref{eq:Inverse_distance_weighting_distance_function_gradient_partial_2}, we obtain the expression for the gradient of the \IDW{} distance function $\forall \boldsymbol{x} \in \mathbb{R}^{n}$, as reported in \eqref{eq:Inverse_distance_weighting_distance_function_gradient}.
\qedwhite{}


% Need this space otherwise the qed symbol is not aligned correctly
